Tackling Compressible Turbulent Multi-Component Flows with Dynamic hp-Adaptation

In this paper, we present an hp-adaptive hybrid Discontinuous Galerkin/Finite Volume method for simulating compressible, turbulent multi-component flows. Building on a previously established hp-adaptive strategy for hyperbolic gas- and droplet-dynamics problems, this study extends the hybrid DG/FV approach to viscous flows with multiple species and incorporates non-conforming interfaces, enabling enhanced flexibility in grid generation. A central contribution of this work lies in the computation of both convective and dissipative fluxes across non-conforming element interfaces of mixed discretizations. To achieve accurate shock localization and scale-resolving representation of turbulent structures, the operator dynamically switches between an h-refined FV sub-cell scheme and a p-adaptive DG method, based on an a priori modal solution analysis. The method is implemented in the high-order open-source framework FLEXI and validated against benchmark problems, including the supersonic Taylor-Green vortex and a triplepoint shock interaction, demonstrating its robustness and accuracy for under-resolved shock-turbulence interactions and compressible multi-species scenarios. Finally, the method's capabilities are showcased through an implicit large eddy simulation of an under-expanded hydrogen jet mixing with air, highlighting its potential for tackling challenging compressible multi-species flows in engineering.

==> Makefile <==
FILENAME='manuscript'

all:
	rubber --unsafe --module lualatex -c 'setlist arguments --shell-escape' -f --pdf -s --synctex --warn=all --jobname=$(FILENAME) $(FILENAME).tex

safe:
	rubber --module lualatex -c 'setlist arguments --shell-escape' -f --pdf -s --warn=all --jobname=$(FILENAME) $(FILENAME).tex

clean:
	ls *.tex | rev | cut -c 5- | rev | xargs rubber --clean

run:
	nohup okular --unique $(FILENAME).pdf\#src:$(LINE)$(FILE) &

